Coresets for Near-Convex Functions

Coreset is usually a small weighted subset of $n$ input points in $\mathbb{R}^d$, that provably approximates their loss function for a given set of queries (models, classifiers, etc.). Coresets become increasingly common in machine learning since existing heuristics or inefficient algorithms may be improved by running them possibly many times on the small coreset that can be maintained for streaming distributed data. Coresets can be obtained by sensitivity (importance) sampling, where its size is proportional to the total sum of sensitivities. Unfortunately, computing the sensitivity of each point is problem dependent and may be harder to compute than the original optimization problem at hand. We suggest a generic framework for computing sensitivities (and thus coresets) for wide family of loss functions which we call near-convex functions. This is by suggesting the $f$-SVD factorization that generalizes the SVD factorization of matrices to functions. Example applications include coresets that are either new or significantly improves previous results, such as SVM, Logistic regression, M-estimators, and $\ell_z$-regression. Experimental results and open source are also provided.

==> relatedWork.tex <==
\section{Related Work}
\label{sec:relatedWork}

\paragraph{Coresets} Given a set $P$ of $n$ points in $\REAL^d$, a (usually infinite) set of queries, and an error parameter $\eps>0$, a coreset $S$ is usually a small (possibly weighted) set of points in $\REAL^d$, such that the answer to every query with respect to $P$, can be $\eps$-approximated by applying it on $S$. In particular, the output of running an existing algorithm on the coreset to compute the optimal query in some sense would yield an approximation to the output of running the same algorithm on the original data, by the definition of the coreset.

Coresets were first suggested in~\cite{AHV04} as a way to improve the theoretical running time of existing algorithms. Today, a coreset is a natural tool for handling Big Data machine learning problems in the streaming and distributed setting. This is mainly due to the merge-and-reduce tree approach that was suggested in~\cite{bentley1980decomposable,sariela}: coresets can be computed independently for subsets of input points, e.g. on different computers, and then can be merged and re-compressed again. Such a binary compression tree can also be computed using one pass over a possibly unbounded streaming set of points, where in every moment only $O(\log n)$ coresets exist in memory for the $n$ point streamed so far. See~\cite{phillips2016coresets} for a recent survey on core-sets.


\paragraph{Machine Learning}
Machine learning problems relies on finding parameters that minimize some objective function. Very often, the objective function is a weighted sum of two terms: a cost function and regularization term. In statistics, the terms are (log-)likelihood and (log-)prior. If both
of these components are convex, then their sum is also convex. Examples of convex optimization problems in machine learning include:

\begin{enumerate}
\item Support Vector Machines(L2-SVM~\cite{suykens1999least}, SVR~\cite{tsang2006generalized}) and Logistic Regression.


\item Regression: linear~\cite{seber2012linear}, sparse linear~\cite{doi:10.1093/biomet/ass043}, ridge~\cite{hoerl1970ridge}, with Tokhonov/$L_1$ regularization~\cite{zarzer2009tikhonov}, and $L_p$~\cite{sposito1982unbiased}.

\item Statistical learning: PageRank~\cite{page1999pagerank}, property testing~\cite{parnas2003testing}, Adaboost~\cite{ratsch2001soft}, D-optimal design~\cite{duchi2011adaptive} and Ellipsoid~\cite{grotschel1981ellipsoid}.

\item Signal processing: e.g. in linear-Gaussian time series or Kalman filters~\cite{hamilton1994time}.

\item Stochastic gradient descent~\cite{chen2006k}, and Frank-Wolfe optimization~\cite{jaggi2013revisiting}.
\end{enumerate}

Most known coresets for support vector machines has relied on reformulating the problem as a MEB (Minimum Enclosing Ball) prbolem; see \cite{clarkson2010coresets,tsang2006generalized} for more details.
As for Logistic Regression, recent work by~\cite{huggins2016coresets}, provided coreset construction method however no bound on the size of the coreset was established. Moreover, a coreset of size polynomial in the dimension and subpolynomial in the number of points (i.e., $\sqrt{n}$ where $n$ is the number of points in a given dataset) was suggested by \cite{munteanu2018coresets} which aimed to convert the problem of Logistic Regression to $L_2$-Regression. The conversion was dependant on the \say{complexity of the data}. However, The formulation of the logistic regression problem at~\cite{munteanu2018coresets} did not include a regularization term. In this paper, we gain similar result to that of~\cite{munteanu2018coresets}, while our formulation of the problem contains a regularization term as well as we have no dependency on the complexity of the data.

As for Regression problems, the notion of well-conditioned basis had been provided by~\cite{dasgupta2009sampling} which esatblished a coreset construction of size independent of number of points and polynomial in the rank of the input matrix, and in this paper, we will follow up on the techniques of~\cite{dasgupta2009sampling} and generalize them to much broader convex functions.
